Useful Evaluation: Syntax and Semantics (Technical Report)

This work provides the first inductive definition of useful CBV evaluation. For that, we first restrict the substitution operation in the Value Substitution Calculus to be linear, yielding the LCBV strategy. We then further restrict substitution in LCBV, so that substitution contributes to the progress of the computation. This optimisation is the UCBV strategy, and its notion of substitution is sensitive to the surrounding evaluation context, so it is non-trivial to capture it inductively. Moreover, we show that UCBV is a sound and complete implementation of LCBV, optimised to implement useful evaluation. As a further contribution, we show that an existing notion of usefulness in the literature, namely the GLAMoUr abstract machine, implements the UCBV strategy with polynomial overhead in time. This establishes that UCBV is time-invariant, i.e., that the number of reduction steps to normal form in UCBV can be used as a measure of time complexity. Defining UCBV leads us to the first semantic model of useful CBV evaluation through system U, a non-idempotent intersection type system. Our main result is a characterisation of termination for useful CBV evaluation via system U: a term is typable in system U if and only if it terminates in UCBV. Additionally, system U provides a quantitative interpretation for UCBV, offering exact step-count information for program evaluation. Even though the specification of the operational semantics of UCBV is highly complex, system U is notably simple. As far as we know, system U is one of the scarce quantitative type systems capturing exactly the substitution step-count for a call-by-value strategy.

==> proofs/compatibile_unfold.tex <==
%Label: lem:compatibile_unfold

\begin{proof}
We prove each item independently.
\begin{enumerate}
\item By induction on the derivation of $\tm \in \HAbs\aset$.
  \begin{itemize}
  \item \ruleHAbsVar.
    Then, $\tm = \var \in \HAbs\aset$ with $\var \in \aset$. 
    Given $\compat\valas\aset\sset$, then $\unvalas\var = \valas(\var)$
    and $\abs{\valas(\var)}$.
  \item \ruleHAbsLam.
    Then, $\tm = \lam\var\tmtwo$. 
    We are done, since $\unvalas{(\lam\var\tmtwo)} = \lam\var\tmtwo$, 
    and $\abs{\lam\var\tmtwo}$ holds.
  \item \ruleHAbsSubi.
    Then, $\tm = \tmtwo\esub\var\tmthree \in \HAbs\aset$ which is 
    derived from $\tmtwo \in \HAbs\aset$ and $\var \notin \aset$.
    Since $\inv\aset\sset{\tmtwo\esub\var\tmthree}$ holds, then it
    implies in particular $\inv\aset{\sset \cup \set\var}\tmtwo$.
    We proceed by showing that 
    $\compat\valas\aset{\sset \cup \set\var}$ holds:
    \begin{itemize}
    \item[(a)]
      Since $\aset \subseteq \dom\valas \subseteq \aset \cup \sset$
      by the hypothesis $\compat\valas\aset\sset$, then 
      $\aset \subseteq \dom\valas \subseteq \aset \cup (\sset \cup \set\var)$.
    \item[(b)]
      Let $\vartwo \in \aset$.
      Since $\inv\aset{\sset \cup \set\var}\tmtwo$ implies 
      $\var \notin \aset$, then $\var \neq \vartwo$ and thus 
      $\abs{\valas(\vartwo)}$ by the hypothesis $\compat\valas\aset\sset$.
    \item[(c)]
      Let $\vartwo \in (\sset \cup \set\var) \cap \dom\valas$. 
      Since $\var \notin \dom\valas$ by $\alpha$-conversion, then 
      $\vartwo \neq \var$. 
      Thus, $\valas(\vartwo)$ is a variable by the hypothesis 
      $\compat\valas\aset\sset$.
    \end{itemize}
    We can now apply the \ih (1) on $\tmtwo$, yielding 
    $\abs{\unvalas\tmtwo}$. We analyse two cases:
    \begin{itemize}
    \item
      If $\unvalas\tmthree = \val\sctx$ and $\var \in \rv\tmtwo$, 
      then $\unvalas{\tmtwo\esub\var\tmthree} = 
      \unvalas[\valas \cup (\var \mapsto \val)]\tmtwo\esub\var\val\sctx$.
      Since $\abs{\unvalas\tmtwo}$ by the \ih (1) on $\tmtwo$, then 
      $\abs{\unvalas[\valas \cup (\var \mapsto \val)]\tmtwo}$ by 
      \cref{rem:abs_valas_abs_valasext}.
      Hence, we conclude with 
      $\abs{\unvalas[\valas \cup (\var \mapsto \val)]\tmtwo\esub\var\val\sctx}$.
    \item
      Otherwise, $\unvalas{\tmtwo\esub\var\tmthree} =
      \unvalas\tmtwo\esub\var{\unvalas\tmthree}$.
      Since $\abs{\unvalas\tmtwo}$ by the \ih (1) on $\tmtwo$, then 
      $\abs{\unvalas\tmtwo\esub\var{\unvalas\tmthree}}$.
    \end{itemize}
  \item 
    \ruleHAbsSubii.
    Then, $\tm = \tmtwo\esub\var\tmthree \in \HAbs\aset$ which is 
    derived from $\tmtwo \in \HAbs{\aset \cup \set\var}$, 
    $\var \notin \aset$, and $\tmthree \in \HAbs\aset$.
    Since $\inv\aset\sset{\tmtwo\esub\var\tmthree}$ holds, then it
    implies both $\inv{\aset \cup \set\var}\sset\tmtwo$ and 
    $\inv\aset\sset\tmthree$.
    Moreover, $\valPred\tmthree$ holds by \cref{rem:habs_st}, so 
    $\unvalas\tmthree = \val\sctx$ by \cref{rem:unfolding_vL}.
    Thus, we analyse two cases, depending on whether 
    $\var \in \rv\tmtwo$ or not:
    \begin{itemize}
    \item
      If $\var \in \rv\tmtwo$, then 
      $\unvalas{\tmtwo\esub\var\tmthree} = 
      \unvalas[\valas \cup (\var \mapsto \val)]\tmtwo\esub\var\val\sctx$.
      Moreover,
      $\compat{\valas \cup (\var \mapsto \val)}{\aset \cup \set\var}\sset$
      holds by \cref{lem:esub_valas_compat_ext_compat} (1).
      Then, 
      $\abs{\unvalas[\valas \cup (\var \mapsto \val)]\tmtwo}$ by the 
      \ih (1) on $\tmtwo$.
      Therefore, $\abs{\unvalas[\valas \cup (\var \mapsto \val)]\tmtwo\esub\var\val\sctx}$.
    \item
      Otherwise, $\unvalas{\tmtwo\esub\var\tmthree} = 
      \unvalas\tmtwo\esub\var{\unvalas\tmthree}$.
      And since $\var \notin \rv\tmtwo$, then
      $\unvalas\tmtwo = \unvalas[\valas \cup (\var \mapsto \val)]\tmtwo$.
      Similarly to the previous case, we obtain 
      $\abs{\unvalas[\valas \cup (\var \mapsto \val)]\tmtwo}$ by the 
      \ih (1) on $\tmtwo$, thus having $\abs{\unvalas\tmtwo}$, so 
      that we can conclude
      $\abs{\unvalas\tmtwo\esub\var{\unvalas\tmthree}}$.
    \end{itemize}
  \end{itemize}
\item By induction on the derivation of $\tm \in \Struct\sset$.
  \begin{itemize}
  \item \ruleStructVar.
    Then, $\tm = \var \in \Struct\sset$ with $\var \in \sset$.
    We analyse two cases depending on whether $\var \in \dom\valas$ or not:
    \begin{itemize}
    \item 
      If $\var \in \dom\valas$, then $\unvalas\var = \valas(\var)$.
      Since $\compat\valas\aset\sset$, then $\valas(\var)$ is a variable.
    \item 
      Otherwise, $\unvalas\var = \var$, so we are done.
    \end{itemize}
  \item \ruleStructApp.
    Then, $\tm = \tmtwo \, \tmthree \in \Struct\sset$.
    This case is not possible, as $\unvalas{(\tmtwo \, \tmthree)} = 
    \unvalas\tmtwo \, \unvalas\tmthree$ is not of the form $\val\sctx$.
  \item \ruleStructSubi.
    Then, $\tm = \tmtwo\esub\var\tmthree \in \Struct\sset$ which is 
    derived from $\tmtwo \in \Struct\sset$ and $\var \notin \sset$.
    We analyse two cases:
    \begin{itemize}
    \item
      If $\unvalas\tmthree = \val_a\sctx_a$ and $\var \in \rv\tmtwo$, 
      then $\unvalas{\tmtwo\esub\var\tmthree} =
      \unvalas[\valas \cup (\var \mapsto \val_a)]\tmtwo\esub\var{\val_a}\sctx_a$.
      Since $\unvalas\tm$ has the form $\val\sctx$, the same holds for 
      $\unvalas[\valas \cup (\var \mapsto \val_a)]\tmtwo$.
      By \cref{lem:valasExt_vL_valas_vL} (2), there exists $\sctx_1$
      such that $\unvalas\tmtwo = \val\sctx_1$.
      Moreover, since $\var \notin \sset$ by hypothesis, we have 
      $\unvalas[\valas \cup (\var \mapsto \val_a)]\vartwo = 
      \unvalas\vartwo$ for all $\vartwo \in \sset$.
      Applying the \ih (2) on $\tmtwo$, we conclude that $\val$ is a 
      variable.
    \item
      Otherwise, $\unvalas{\tmtwo\esub\var\tmthree} =
      \unvalas\tmtwo\esub\var{\unvalas\tmthree}$.
      Since $\unvalas\tm$ is of the form $\val\sctx$, the same holds
      for $\unvalas\tmtwo$.
      Following the same reasoning from case \ruleHAbsSubi in the 
      previous item, $\compat\valas\aset{\sset \cup \set\var}$ holds.
      Moreover, $\tmtwo \in \Struct{\sset \cup \set\var}$ by 
      \cref{rem:habs_st}.
      Since $\inv\aset\sset{\tmtwo\esub\var\tmthree}$ implies in 
      particular $\inv\aset{\sset \cup \set\var}\tmtwo$, we can then 
      apply the \ih (2) on $\tmtwo$, yielding that $\val$ is a variable.
    \end{itemize}
  \item 
    \ruleStructSubii.
    Then $\tm = \tmtwo\esub\var\tmthree \in \Struct\sset$ which is 
    derived from $\tmtwo \in \Struct{\sset \cup \set\var}$,
    $\var \notin \sset$, and $\tmthree \in \Struct\sset$.
    Since $\inv\aset\sset{\tmtwo\esub\var\tmthree}$ holds, then it
    implies in particular $\inv\aset{\sset \cup \set\var}\tmtwo$.
    Moreover, $\compat{\valas'}\aset{\sset \cup \set\var}$ holds by 
    \cref{lem:esub_valas_compat_ext_compat} (2), where 
    $\valas' = \valas \cup (\var \mapsto \val_a)$ if 
    $\var \in \rv\tmtwo$ and $\unvalas\tmthree = \val_a\sctx_a$, for 
    some $\val_a$, $\sctx_a$, or $\valas' = \valas$ otherwise.
    Since $\unvalas\tm$ is of the form $\val\sctx$, the same holds 
    for $\unvalas[\valas']\tmtwo$.
    We can then apply the \ih (2) on $\tmtwo$, yielding that $\val$ 
    is a variable.
  \end{itemize}
\end{enumerate}
\end{proof}


==> proofs/normal_forms_zero_counter.tex <==
% Label: lem:normal_forms_zero_counter

\begin{proof}
By induction on the derivation of $\tm \in \NF{\aset}{\sset}{\appflag}$.
\begin{enumerate}
  \item \ruleUNFVar.
    The following conditions hold:
    \begin{enumerate}
    \item[(a)]
      \[
        \indrule{\ruleUNFVar}{
          \var \in \aset \implies \appflag = \nonapp
        }{
          \var \in \NF{\aset}{\sset}{\appflag}
        }
      \]
    \item[(b)] $\judg[m,e]{\tctx}{\var}{\tight}$ is tight
    \item[(c)] $\isAppr{\aset}{\tctx}$
    \item[(d)] If $\appflag = \app$ then $\tight = \tightN$.
    \end{enumerate}
    The judgment of the condition (b) can only be derived by rule \ruleTypVar,
    so
    \[
     \judg[0, \numarrows{\tight}]{\var : \tight}{\var}{\tight}
    \]
    with $\tctx = \var : \tight, m = 0$ and
   $e = \numarrows{\tight} =0$.
    We conclude immediately.
  \item \ruleUNFLam.
    The following conditions hold:
    \begin{enumerate}
    \item[(a)]
      \[
        \indrule{\ruleUNFLam}{}{
          \lam{\var}{\tmtwo} \in \NF{\aset}{\sset}{\nonapp}
        }
      \]
    \item[(b)] $\judg[m,e]{\tctx}{\lam{\var}{\tmtwo}}{\tight}$ is tight
    \item[(c)] $\isAppr{\aset}{\tctx}$
    \item[(d)] Here $\appflag = \nonapp$.
    \end{enumerate}
    The judgment of  condition (b) can only be derived  by rule \ruleTypAbs.
    Moreover, the only possible case where
    this judgment is tight is when
    the resulting type of the abstraction is $\mset$, which holds with no premises:
    \[
      \indrule{\ruleTypAbs}{}{
        \judg[0, 0]{\emptyctx}{\lam{\var}{\tmtwo}}{\emset}
      }
    \]
    So we can conclude that the counters are $(0, 0)$.
  \item \ruleUNFApp.
    The following conditions hold:
    \begin{enumerate}
    \item[(a)]
      \[
        \indrule{\ruleUNFApp}{
          \tmtwo \in \NF{\aset}{\sset}{\app}
          \sep
          \tmthree \in \NF{\aset}{\sset}{\nonapp}
        }{
          \tmtwo\,\tmthree \in \NF{\aset}{\sset}{\appflag}
        }
      \]
    \item[(b)] $\judg[m,e]{\tctx}{\tmtwo\,\tmthree}{\tight}$ is tight
    \item[(c)] $\isAppr{\aset}{\tctx}$
    \item[(d)] If $\appflag = \app$ then $\tight = \tightN$.
    \end{enumerate}
    The judgment of  condition (b) 
    can be derived either by rule \ruleTypAppP\ or rule \ruleTypAppC.
    \begin{enumerate}
    \item \ruleTypAppP.
      Then
      \[
        \indrule{\ruleTypAppP}{
          \judg[m_1,e_1]{\tctx_1}{\tmtwo}{\tightN}
          \sep
          \judg[m_2,e_2]{\tctx_2}{\tmthree}{\tight}
        }{
          \judg[m_1 + m_2,e_1 + e_2]{\tctx_1 + \tctx_2}{\tmtwo\,\tmthree}{\tightN}
        }
      \]
      with $\tctx = \tctx_1 + \tctx_2, m = m_1 + m_2, e = e_1 + e_2$ and $\tight = \tightN$.
      The following conditions hold:
      \begin{enumerate}
      \item[(a')] $\tmtwo \in \NF{\aset}{\sset}{\app}$ by condition (a)
      \item[(b')] $\judg[m_1,e_1]{\tctx_1}{\tmtwo}{\tightN}$ 
        is tight since $\tctx = \tctx_1 + \tctx_2$, and $\tctx$ is tight by condition (b)
      \item[(c')] $\isAppr{\aset }{\tctx_1}$, since $\tctx = \tctx_1 + \tctx_2$ and
        $\isAppr{\aset }{\tctx}$ by condition (c)
      \item[(d')] It holds that $\appflag = \app$, and the term $\tmtwo$ is typed with $\tightN$. 
      \end{enumerate}
      We can apply \ih on $\tmtwo$, yielding $(m_1, e_1) = (0,0)$.      
      On the other hand, the following conditions hold:
      \begin{enumerate}
      \item[(a'')] $\tmthree \in \NF{\aset}{\sset}{\nonapp}$, by condition (a)
      \item[(b'')] $\judg[m_2,e_2]{\tctx_2}{\tmthree}{\tight}$ is tight
        since $\tctx = \tctx_1 + \tctx_2$,
        and $\tctx$ is tight by condition (b)
      \item[(c'')] $\isAppr{\aset}{\tctx_2}$, since $\tctx = \tctx_1 + \tctx_2$ and 
        $\isAppr{\aset }{\tctx}$ by condition (c)
      \item[(d'')] Here $\appflag \neq \app$.
      \end{enumerate}
      We can apply \ih on $\tmthree$, yielding $(m_2, e_2) = (0,0)$.
      Then, we can conclude that $(m_1 + m_2, e_1 + e_2) = (0, 0)$.
    \item \ruleTypAppC.
      Then we have:
      \[
        \indrule{\ruleTypAppC}{
          \judg[m_1,e_1]{\tctx_1}{\tmtwo}{\mset{\optmtyp \to \tight}}
          \sep
          \optmtyp \mleq \mtyp
          \sep
          \judg[m_2,e_2]{\tctx_2}{\tmthree}{\mtyp}
        }{
          \judg[1 + m_1 + m_2,e_1 + e_2]{\tctx_1 + \tctx_2}{\tmtwo\,\tmthree}{\tight}
        }
      \]
      with $\tctx = \tctx_1 + \tctx_2, m = 1 + m_1 + m_2$ and $e = e_1
      + e_2$.
      We have $\tmtwo \in \Struct{\sset}$
      by \cref{lem:nf_in_HAbs_or_Struct}.
      Moreover, $\tctx_1$ is tight since $\tctx = \tctx_1 + \tctx_2$,
      and $\tctx$ is tight.
      Furthermore, $\inv{\aset}{\sset}{\tm}$ implies $\inv{\aset}{\sset}{\tmtwo}$.
     We can then apply 
      \cref{lem:tight_spreading_struct}, yielding that the singleton
      $\mset{\optmtyp \to \tight}$ must be tight, which is impossible.
      Hence this case does not apply.
    \end{enumerate}
  \item \ruleUNFEsAbs.
    The following conditions hold:
    \begin{enumerate}
    \item[(a)]
      \[
        \indrule{\ruleUNFEsAbs}{
          \tmtwo \in \NF{\aset \cup \set{\var}}{\sset}{\appflag}
          \sep
          \tmthree \in \NF{\aset}{\sset}{\nonapp}
          \sep
          \tmthree \in \HAbs{\aset}
        }{
          \tmtwo\esub{\var}{\tmthree} \in \NF{\aset}{\sset}{\appflag}
        }
      \]
    \item[(b)] $\judg[m,e]{\tctx}{\tmtwo\esub{\var}{\tmthree}}{\tight}$ is tight
    \item[(c)] $\isAppr{\aset}{\tctx}$
    \item[(d)] If $\appflag = \app$ then $\tight = \tightN$.
    \end{enumerate}
    The judgment of  condition (b) 
    can be derived only by rule \ruleTypES, so
    \[
      \indrule{\ruleTypES}{
        \judg[m_1,e_1]{\tctx_1; \var : \optmtyp}{\tmtwo}{\tight}
        \sep
        \optmtyp \mleq \mtyp
        \sep
        \judg[m_2,e_2]{\tctx_2}{\tmthree}{\mtyp}
      }{
        \judg[m_1 + m_2,e_1 + e_2]{\tctx_1 + \tctx_2}{\tmtwo\esub{\var}{\tmthree}}{\tight}
      }
    \]
    where $\tctx = \tctx_1 + \tctx_2, m = m_1 + m_2$ and $e = e_1 + e_2$.
    We may assume $\var \notin (\aset \cup \sset)$
    by Barendregt's convention.
    There are two cases, depending on whether $\mtyp$ is tight or not:
    \begin{enumerate}
    \item $\mtyp = \tight$.
      The following conditions hold:
      \begin{enumerate}
      \item[(a')] $\tmtwo \in \NF{\aset \cup \set{\var}}{\sset}{\appflag}$, by condition (a)
      \item[(b')] $\judg[m_1,e_1]{\tctx_1; \var : \optmtyp}{\tmtwo}{\tight}$
        is tight. Indeed,  
        \begin{enumerate}
        \item[(1)] $\tctx_1$ is tight because  $\tctx = \tctx_1 + \tctx_2$ and condition (b); 
        \item[(2)] $\optmtyp$ is tight since $\mtyp$ is tight and $\optmtyp \mleq \mtyp$; 
        \item[(3)] the type of the term is $\tightN$.
        \end{enumerate}
      \item[(c')] $\isAppr{\aset \cup \set{\var}}{\tctx_1; \var : \optmtyp}$.
        Indeed,
        \begin{enumerate}
        \item[(1)]  $\isAppr{\aset}{\tctx_1}$ holds because 
        $\tctx = \tctx_1 + \tctx_2$, and condition (c), thus  $\isAppr{\aset\cup \set{\var}}{\tctx_1}$
        by \cref{rem:isAppropriate};   
        
        \item[(2)]  $\tmthree \in \HAbs{\aset}$ holds by condition (a) and
        $\isAppr{\aset}{\tctx_1}$ holds because 
        $\tctx = \tctx_1 + \tctx_2$ and $\isAppr{\aset}{\tctx}$
        by condition (c). Then 
        $\tight \neq \tightN$ by \cref{lem:types_of_hereditary_abstractions}
        (so also $\optmtyp \neq \tightN$), thus
        $\isAppr{\aset \cup \set{\var}}{\var : \optmtyp}$. 
        \end{enumerate}
      \item[(d')] If $\appflag = \app$ then $\tight = \tightN$ by condition (d).
      \end{enumerate}
      We can apply \ih on $\tmtwo$, yielding $(m_1, e_1) = (0,0)$.
      On the other hand, the following conditions hold:
      \begin{enumerate}
      \item[(a'')] $\tmthree \in \NF{\aset}{\sset}{\nonapp}$, by condition (a)
      \item[(b'')] $\judg[m_2,e_2]{\tctx_2}{\tmthree}{\mtyp}$ is tight. Indeed,
        \begin{enumerate}
        \item[(1)] $\tctx_2$ is tight because  $\tctx = \tctx_1 + \tctx_2$ and
          condition (b);
         \item[(2)] $\mtyp$ is tight by hypothesis.
        \end{enumerate}
      \item[(c'')] $\isAppr{\aset}{\tctx_2}$ holds because  $\tctx = \tctx_1 + \tctx_2$ and  condition (c); 
      \item[(d'')] Here $\appflag \neq \app$.
      \end{enumerate}
      We can apply \ih on $\tmthree$, yielding $(m_2, e_2) = (0,0)$.
      Then, we can conclude that $(m_1 + m_2, e_1 + e_2) = (0, 0)$.
    \item $\mtyp \neq \tight$.
      Then $\optmtyp$ cannot be $\none$. 
      Moreover, $\optmtyp = \mtyp$ and they are non-empty multisets,
      since $\mtyp = \emset$ would be tight.
      Hence the following conditions hold:
      \begin{enumerate}
      \item[(1)] $\judg[m_1,e_1]{\tctx_1; \var : \optmtyp}{\tmtwo}{\tight}$ is derivable by condition (a); 
      \item[(2)] $\isAppr{\aset \cup \set{\var}}{\tctx_1}$, since 
        (2.1) $\var \notin \dom{\tctx_1}$, and
        (2.2) $\tctx = \tctx_1 + \tctx_2$ and condition (c).
        It also holds that $\tctx_1$ is tight by $\tctx = \tctx_1 + \tctx_2$
        and condition (b); 
      \item[(3)] $\var:\optmtyp \neq \emptyctx$, as argued; 
      \item[(4)] $\dom{\var : \mtyp} = \set{\var} \subseteq \aset \cup \set{\var}$
      \item[(5)] For all $\vartwo \in \dom{\var : \mtyp}$, we have that $(\var : \mtyp)(\vartwo)=\mtyp$ is a non-empty multiset.
      \end{enumerate}
      Moreover, $\inv{\aset}{\sset}{\tmtwo\esub{\var}{\tmthree}}$ implies $\inv{\aset \cup \set{\var}}{\sset}{\tmtwo}$.
      Then 
      $\tmtwo \notin \NF{\aset \cup \set{\var}}{\sset}{\appflag}$
      by \cref{lem:reducible_when_multisets},
      which contradicts condition (a).
      Hence this case is not possible.
    \end{enumerate}
  \item \ruleUNFEsStruct.
    The following conditions hold:
    \begin{enumerate}
    \item[(a)]
      \[
        \indrule{\ruleUNFEsStruct}{
          \tmtwo \in \NF{\aset}{\sset \cup \set{\var}}{\appflag}
          \sep
          \tmthree \in \NF{\aset}{\sset}{\nonapp}
          \sep
          \tmthree \in \Struct{\sset}
        }{
          \tmtwo\esub{\var}{\tmthree} \in \NF{\aset}{\sset}{\appflag}
        }
      \]
    \item[(b)] $\judg[m,e]{\tctx}{\tmtwo\esub{\var}{\tmthree}}{\tight}$ is tight
    \item[(c)] $\isAppr{\aset}{\tctx}$
    \item[(d)] If $\appflag = \app$ then $\tight = \tightN$.
    \end{enumerate}
    The judgment of  condition (b) 
    can only be derived  by rule \ruleTypES, so
    \[
      \indrule{\ruleTypES}{
        \judg[m_1,e_1]{\tctx_1; \var : \optmtyp}{\tmtwo}{\tight}
        \sep
        \optmtyp \mleq \mtyp
        \sep
        \judg[m_2,e_2]{\tctx_2}{\tmthree}{\mtyp}
      }{
        \judg[m_1 + m_2,e_1 + e_2]{\tctx_1 + \tctx_2}{\tmtwo\esub{\var}{\tmthree}}{\tight}
      }
    \]
    where $\tctx = \tctx_1 + \tctx_2, m = m_1 + m_2$ and $e = e_1 + e_2$.
    By condition (b) $\tctx$ is tight, 
    so it must hold in particular that $\tctx_2$ is $\sset-$tight.
    Then  $\tmthree \in \Struct{\sset}$ implies that $\mtyp$ must be tight by \cref{lem:tight_spreading_struct}.
    Hence the following conditions hold:
    \begin{enumerate}
    \item[(a')] $\tmthree \in \NF{\aset}{\sset}{\nonapp}$, by condition (a)
    \item[(b')] $\judg[m_2,e_2]{\tctx_2}{\tmthree}{\mtyp}$ is tight since
      (1) $\tctx = \tctx_1 + \tctx_2$ and condition (b); 
      (2) $\mtyp$ is tight
    \item[(c')] $\isAppr{\aset}{\tctx_2}$, since $\tctx = \tctx_1 + \tctx_2$ and condition (c)
    \item[(d')] Here $\appflag = \nonapp$.
    \end{enumerate}
    We can apply \ih on $\tmthree$, yielding $(m_2, e_2) = (0, 0)$.
    On the other hand, 
    we may assume $\var \notin \aset \cup \sset$ by Barendregt's convention. 
    Moreover,
    $\inv{\aset}{\sset}{\tmtwo\esub{\var}{\tmthree}}$ implies $\inv{\aset}{\sset \cup \set{\var}}{\tmtwo}$.
    The following conditions holds:
    \begin{enumerate}
    \item[(a'')] $\tmtwo \in \NF{\aset}{\sset \cup \set{\var}}{\appflag}$, by condition (a)
    \item[(b'')] $\judg[m_1,e_1]{\tctx_1; \var : \optmtyp}{\tmtwo}{\tight}$
      is tight. Indeed, 
      \begin{enumerate}
        \item[(1)] the resulting type is tight,
      \item[(2)] $\tctx_1$ is tight since $\tctx = \tctx_1 + \tctx_2$ and  condition (b), and
      \item[(3)] $\var : \optmtyp$ is tight since $\optmtyp \mleq \mtyp$, 
      and $\mtyp$ is tight so $\optmtyp$ must be $\none$ or tight
      \end{enumerate}
    \item[(c'')] $\isAppr{\aset}{\tctx_1; \var : \optmtyp}$, since $\var \notin \aset$ and
      $\tctx = \tctx_1 + \tctx_2$, and  condition (c)
    \item[(d'')] If $\appflag = \app$, then $\tight = \tightN$, by condition (d).
    \end{enumerate}
   We can apply \ih on $\tmtwo$ yielding $(m_1, e_1) = (0, 0)$.
    Then, we can conclude that $(m_1 + m_2, e_1 + e_2) = (0, 0)$, so we are done.

\end{enumerate}
\end{proof}



==> proofs/splitting_ctx_nf.tex <==
% Label: lem:splitting_ctx_nf

\begin{proof}
We prove both implications by structural induction on $\sctx$.

We first show that $\tm\sctx \in \VNF{\vset}{\appflag}$ implies
$\tm \in \VNF{\expansion{\vset}{\sctx}}{\appflag}$ and $\sctx \in \CtxNF{\vset}$:
\begin{enumerate}
\item $\sctx = \ctxhole$.
  Then $\expansion{\vset}{\ctxhole} = \vset$ by definition.
  We conclude $\tm \in \VNF{\vset}{\appflag}$ by hypothesis,
  and $\ctxhole \in \CtxNF{\vset}$ by rule \ruleCtxNFEmpty.
\item $\sctx = \sctx'\esub{\var}{\tmtwo}$.
  We have to analyze two cases:
  \begin{enumerate}
  \item[(a)] $\valPred{\tmtwo}$.
    Then
    $\tm\sctx'\esub{\var}{\tmtwo} \in \VNF{\vset}{\appflag}$
    is derived from rule \ruleVNFEsVal,
    with $\tm\sctx' \in \VNF{\vset \cup \set{\var}}{\appflag}$
    and $\tmtwo \in \VNF{\vset}{\nonapp}$.
    By \ih on $\sctx'$, we have that
    $\tm \in 
     \VNF{\expansion{(\vset \cup \set{\var})}{\sctx'}}{\appflag}$
    and $\sctx' \in \CtxNF{\vset \cup \set{\var}}$,
    where
    $ \expansion{(\vset \cup \set{\var})}{\sctx'}
    = \expansion{\vset}{\sctx'} \cup \set{\var}
    = \expansion{\vset}{\sctx'\esub{\var}{\tmtwo}}
    $
    by definition,
    since we may assume 
    $\var \notin \domSctx{\sctx'}$ by Barendregt's convention.
    Applying rule $\ruleCtxNFAddVal$ we conclude
    $\sctx'\esub{\var}{\tmtwo} \in \CtxNF{\vset}$.
  \item[(b)] $\neg(\valPred{\tmtwo}).$ % Análogo al caso anterior.
    Then
    $\tm\sctx'\esub{\var}{\tmtwo} \in \VNF{\vset}{\appflag}$
    is derived from rule \ruleVNFEsNonVal,
    with $\tm\sctx' \in \VNF{\vset}{\appflag}$
    and $\tmtwo \in \VNF{\vset}{\nonapp}$.
    By \ih on $\sctx'$, we have that
    $\tm \in \VNF{\expansion{\vset}{\sctx'}}{\appflag}$
    and $\sctx' \in \CtxNF{\vset}$,
    where
    $ \expansion{\vset}{\sctx'\esub{\var}{\tmtwo}} 
    = \expansion{\vset}{\sctx'}$
    by definition.
    Applying rule $\ruleCtxNFAddNonVal$ we conclude
    $\sctx'\esub{\var}{\tmtwo} \in \CtxNF{\vset}$.
  \end{enumerate}
\end{enumerate}
We now show that $\tm \in \VNF{\expansion{\vset}{\sctx}}{\appflag}$ and 
$\sctx \in \CtxNF{\vset}$ implies $\tm\sctx \in \VNF{\vset}{\appflag}$:
\begin{enumerate}
\item $\sctx = \ctxhole$.
  Immediate.
\item $\sctx = \sctx'\esub{\var}{\tmtwo}$.
  Then
  $\tm \in \VNF{\expansion{\vset}{\sctx'\esub{\var}{\tmtwo}}}{\appflag}$
  and
  $\sctx'\esub{\var}{\tmtwo} \in \CtxNF{\vset}$.
  We have to analyze two cases,
  depending on which rule is used to derive the former judgment:
  \begin{enumerate}
  \item[(a)] $\ruleCtxNFAddVal$.
    Then the premises are
    $\sctx' \in \CtxNF{\vset \cup \set{\var}}$,
    $\tmtwo \in \VNF{\vset}{\nonapp}$,
    and $\valPred{\tmtwo}$, so
    $ \expansion{\vset}{\sctx'\esub{\var}{\tmtwo}} 
    = \expansion{\vset}{\sctx'} \cup \set{\var}$
    by definition. Therefore
    $\tm \in \VNF{\expansion{(\vset \cup \set{\var})}{\sctx'}}{\appflag}$,
    since we may assume
    $\var \notin \sctx'$ by Barendregt's convention.
    By \ih on $\sctx'$,
    we have that
    $\tm\sctx' \in \VNF{\vset \cup \set{\var}}{\appflag}$.
    We can apply rule $\ruleVNFEsVal$,
    yielding $\tm\sctx'\esub{\var}{\tmtwo} \in \VNF{\vset}{\appflag}$.
  \item[(b)] $\ruleCtxNFAddNonVal$. % Análogo al caso anterior.
    Then
    $\sctx' \in \CtxNF{\vset}$,
    $\tmtwo \in \VNF{\vset}{\nonapp}$,
    and $\neg(\valPred{\tmtwo})$, so
    $ \expansion{\vset}{\sctx'\esub{\var}{\tmtwo}} 
    = \expansion{\vset}{\sctx'}$
    by definition, therefore
    $\tm \in \VNF{\expansion{\vset}{\sctx'}}{\appflag}$.
    By \ih on $\sctx'$,
    we have that
    $\tm\sctx' \in \VNF{\vset}{\appflag}$.
    We can apply rule $\ruleVNFEsNonVal$,
    yielding $\tm\sctx'\esub{\var}{\tmtwo} \in \VNF{\vset}{\appflag}$.
  \end{enumerate}
\end{enumerate}
\end{proof}

